Multilingual Amnesia: On the Transferability of Unlearning in Multilingual LLMs

As multilingual large language models become more widely used, ensuring their safety and fairness across diverse linguistic contexts presents unique challenges. While existing research on machine unlearning has primarily focused on monolingual settings, typically English, multilingual environments introduce additional complexities due to cross-lingual knowledge transfer and biases embedded in both pretraining and fine-tuning data. In this work, we study multilingual unlearning using the Aya-Expanse 8B model under two settings: (1) data unlearning and (2) concept unlearning. We extend benchmarks for factual knowledge and stereotypes to ten languages through translation: English, French, Arabic, Japanese, Russian, Farsi, Korean, Hindi, Hebrew, and Indonesian. These languages span five language families and a wide range of resource levels. Our experiments show that unlearning in high-resource languages is generally more stable, with asymmetric transfer effects observed between typologically related languages. Furthermore, our analysis of linguistic distances indicates that syntactic similarity is the strongest predictor of cross-lingual unlearning behavior.

==> extra.tex <==
% In this work, we address the problem of multilingual unlearning by distinguishing between two key categories of information to be forgotten: (1) \textit{fine-tuned knowledge} and (2) \textit{biases inherited from pretraining corpora}. 
% Using the TOFU and SeeGULL datasets translated into English, French, Hindi, Arabic, and Farsi, we demonstrate that unlearning targeted content in one language generally results in minimal performance degradation in others. However, partial propagation occurs, particularly between typologically similar or high-resource languages such as English and French. 
% These findings underscore the need for language-aware unlearning strategies and the development of multilingual safety benchmarks that account for shared context and cross-lingual transfer effects.


% As multilingual large language models become increasingly prevalent, ensuring their safety and fairness across languages presents new challenges. While most machine unlearning research has focused on monolingual contexts, multilingual settings introduce unique complexities due to cross-lingual knowledge transfer and entrenched biases in both pretraining and fine-tuning data. In this work, we address the problem of multilingual unlearning by distinguishing between two key categories of information to be forgotten: (1) \textit{fine-tuned knowledge}—such as stereotypes introduced during downstream training—and (2) \textit{biases inherited from pretraining corpora}. We perform unlearning multilingual scenarios using the TOFU and SeeGULL datasets, translated into English, French, Hindi, Arabic, and Farsi. Our experiments demonstrate that unlearning targeted content in one language typically results in minimal performance degradation in others. However, partial propagation is observed, particularly between typologically or resource-similar languages like English and French. These findings highlight the need for language-aware unlearning strategies and the development of multilingual safety benchmarks that account for shared context and cross-lingual transfer effects.


% This task is known as \textbf{machine unlearning} and centers on deleting individual data points while preserving the model’s remaining knowledge \citep{bourtoule2021machine, zhang2024rightforgotteneralarge}.
% A separate challenge is eliminating broader unsafe or harmful content that the model has absorbed during pre-training, such as nationality-based slurs, self-harm instructions, or recipes for chemical weapons. Removing these high-level behaviors—often called \textbf{concept unlearning}—is motivated by safety and harm-reduction rather than privacy \citep{liu2024rethinkingmachineunlearninglarge}.
% Together, machine and concept unlearning provide complementary tools: the former enforces privacy compliance at the data-point level, while the latter mitigates harmful or dangerous behaviors embedded in the model’s general knowledge \citep{Jaman, NEURIPS2023_2ecc8008}.

% 
% Whenever these models memorize private facts, amplify defamation, or encode harmful stereotypes, developers must be able to delete that information quickly, reliably, and without the prohibitive cost of full retraining \citep{zhang2024rightforgotteneralarge}. This imperative, rooted in regulations such as the EU’s “Right to be Forgotten” and in growing safety concerns, has given rise to the field of machine unlearning: methods that remove selected knowledge while preserving the rest of the model’s capabilities. Early work on machine unlearning focused on efficiently excising particular training examples or data points from models \citep{bourtoule2021machine}. Since then, the scope of unlearning has expanded to include removing broader, potentially harmful concepts that a model may have inadvertently learned. In parallel, ensuring that LLMs avoid undesirable or unsafe behaviors, such as perpetuating cultural stereotypes learned during pretraining, has become a major challenge \citep{liu2024rethinkingmachineunlearninglarge}. Unlearning, therefore, plays a dual role: enabling \textit{privacy} (by removing personal or factual content) and promoting \textit{fairness} (by mitigating harmful social biases \citealp{Jaman, NEURIPS2023_2ecc8008}).
% In this paper, we take the first step towards filling that gap. We ask two concrete questions:
% \begin{itemize}
%     \item \textbf{RQ1:} If we unlearn something in one language, does it also disappear in other languages within the same multilingual model?
%     \item \textbf{RQ2:} How does the effect of unlearning vary across languages and types of information (fine-tuned vs. pretrained)? Is cross-lingual propagation more likely between linguistically similar or high-resource languages?
% \end{itemize}
% These questions matter not only for model safety, but also for efficient intervention. If forgetting generalizes across languages, we can apply targeted unlearning in just one or two languages. If not, multilingual unlearning requires language-specific solutions.

% To address these questions, we conduct two complementary experiments that correspond to the data and concept unlearning settings which we define in the Section~\ref{sec:methodology}.
% \begin{itemize}
%     \item \textbf{Data Unlearning}. To evaluate the removal of individual sensitive data points, we utilize the privacy-oriented TOFU benchmark \citep{tofu2024}, originally designed to assess factual unlearning in English. We extend this benchmark to four additional languages (French, Hindi, Arabic, and Farsi). This language set help us analysis how typological similarity (e.g., English–French) and resource availability (e.g., low-resource Farsi) influence the transferability of unlearning effects in multilingual LLMs.
%     \item \textbf{Concept Unlearnin}g. We assess the deletion of broader harmful concepts with a question-answering adaptation of SeeGULL \cite{jha-etal-2023-seegull} stereotype corpus, chosen for its fine-grained coverage of nationally anchored stereotypes.
%     % We release multilingual versions in English, French, and Hindi to capture both high- and mid-resource scenarios.
% \end{itemize}

% We propose the first framework to evaluate the transferability of unlearning in multilingual LLMs, addressing two key scenarios, machine unlearning and concept unlearning.
% \item \textbf{Multilingual Extension of Unlearning Benchmarks}: We extend two established unlearning benchmarks, TOFU and SeeGULL, to support multilingual evaluation across 5 languages. Our evaluation includes [human-verified translations / quality control] to ensure the reliability of multilingual data to enable accurate assessment of unlearning transferability across languages. (Clarify the annotation status here, if there’s no human annotation, we should not claim the translation quality or creation of the multilingual benchmark as a contribution.)


% To answer these questions, we study multilingual unlearning in LLMs by examining two distinct types of information:
% (1) Fine-tuned knowledge and
% (2) Pretraining-derived biases.
% For empirical analysis, we construct two complementary testbeds: a multilingual adaptation of the TOFU factual-forgetting benchmark (English, French, Hindi, Arabic, Farsi) and a question-answering version of the geo-cultural SeeGULL stereotype dataset. We then apply a gradient-ascent unlearning procedure that down-weights the probability of undesirable answers while maintaining performance on held-out data, and we measure cross-lingual effects on Aya-Expanse-8B and Llama-3.1-8B-Instruct.

% In this work, we study multilingual unlearning in LLMs by examining two distinct types of information: (1) \textit{fine-tuned knowledge}, such as stereotypes introduced during downstream training; and (2) \textit{biases inherited from pretraining data}, which are harder to localize and remove. We employ Gradient Ascent (GA) based approaches for unlearning, which allow us to target undesirable behaviors while preserving unrelated capabilities. To analyze cross-lingual effects, we use two multilingual datasets: the TOFU dataset \citep{tofu2024} for fact unlearning (translated into French, Hindi, Arabic, and Farsi), and an adapted version of the SeeGULL dataset \citep{jha-etal-2023-seegull} for stereotype unlearning across English, French, and Hindi. 
% % The SeeGULL dataset contains over 7,000 stereotypes from 178 countries, enabling us to probe geoculturally situated bias representations across languages.
% In our study we address the following research questions:
% \begin{itemize}
%     \item \textbf{RQ1:} Does unlearning in one language affect the same content in others? That is, is unlearning in one language sufficient to remove the corresponding information from the multilingual model?
%     \item \textbf{RQ2:} How does the effect of unlearning vary across languages and types of information (fine-tuned vs. pretrained)? Is cross-lingual propagation more likely between linguistically similar or high-resource languages?
% \end{itemize}

% These questions matter not only for model safety, but also for efficient intervention. If forgetting generalizes across languages, we can apply targeted unlearning in just one or two languages. If not, multilingual unlearning requires language-specific solutions.

% Our contributions are summarized as follows:
% \begin{itemize}
%     \item We present one of the \textbf{first} systematic studies of cross-lingual unlearning in multilingual LLMs, examining how unlearning in one language affects others.
%     % (Figure~\ref{fig:main})
%     \item We distinguish between fine-tuned knowledge and pretraining biases, showing they behave differently under unlearning interventions.
%     \item We adapt and utilize multilingual versions of the TOFU and SeeGULL datasets to support evaluation across privacy and fairness contexts.
%     \item We find that unlearning effects are often language-specific but can partially propagate between closely related or high-resource languages, such as English and French.
% \end{itemize}


% Recent advances in machine unlearning (MU) have shown promising potential for both privacy protection and bias mitigation in LLMs \citep{NEURIPS2023_2ecc8008, alsharabi}. Broadly, MU refers to the process of selectively removing training-induced knowledge such that the model behaves as if specific data were never seen. Initially introduced by \citet{cao}, the concept has evolved through techniques like sharded retraining, most notably the SISA framework, which enables efficient data deletion without full model retraining \citep{bourtoule2021machine} and selective forgetting via controlled parameter updates \citep{golatkar2020eternalsunshinespotlessnet}.

% More recently, MU has been applied to LLMs through two main approaches: fine-tuning-based unlearning such as gradient ascent to erase copyrighted or sensitive content \citep{eldan2023whosharrypotterapproximate, chen2023unlearnwantforgetefficient} and direct parameter editing via methods like weight surgery or subspace pruning \citep{meng2023locatingeditingfactualassociations, lizzo2024unlearnefficientremovalknowledge}. Additionally, \citet{Zhang2024-yo} demonstrate that unlearning biased data points can be achieved without introducing new biases, emphasizing MU’s potential for fairness. \citet{NEURIPS2023_2ecc8008} further propose a counterfactual unlearning approach using influence functions and minimal parameter updates to reduce the cost of retraining. Complementary to these, \citet{Yuanshun} show that using negative examples where models are fine-tuned to assign low likelihoods to harmful/undesired outputs, can outperform RLHF in safety alignment tasks, offering a more computationally efficient alternative.

% In recent years, MU has been extended to LLMs, giving rise to two main methodological paradigms: (1) fine-tuning-based unlearning, and (2) parameter-specific editing. In the first approach, models are subjected to additional fine-tuning that reverses or overwrites learned representations. For example, gradient ascent has been used to make models forget copyrighted material or sensitive information without requiring full retraining \citep{eldan2023whosharrypotterapproximate, chen2023unlearnwantforgetefficient}. In contrast, parameter-editing methods aim to directly identify and modify the weights responsible for encoding specific facts or behaviors. Techniques such as weight surgery and knowledge-subspace pruning have been proposed to surgically remove unwanted information while preserving general model performance \citep{meng2023locatingeditingfactualassociations, lizzo2024unlearnefficientremovalknowledge}.



%##############################


% Machine unlearning (MU) aims to remove the influence of specific training data from a model, ensuring it behaves as if that data were never seen \citep{cao}. Early frameworks such as SISA introduced sharded retraining for efficient data deletion \citep{bourtoule2021machine}, while later work proposed selective forgetting via parameter updates \citep{golatkar2020eternalsunshinespotlessnet}. More recently, MU has been applied to LLMs through two main approaches: fine-tuning-based unlearning such as gradient ascent to erase copyrighted or sensitive content \citep{eldan2023whosharrypotterapproximate, chen2023unlearnwantforgetefficient} and direct parameter editing via methods like weight surgery or subspace pruning \citep{meng2023locatingeditingfactualassociations, lizzo2024unlearnefficientremovalknowledge}.

% These strategies have shown promise in mitigating bias and enhancing safety. For instance, counterfactual unlearning based on influence functions has enabled low-cost updates with minimal side effects \citep{NEURIPS2023_2ecc8008}, while others leverage negative examples to suppress harmful outputs more efficiently than RLHF \citep{Yuanshun}. Further, unlearning biased samples without introducing new biases has been demonstrated as a pathway to fairer model behavior \citep{Zhang2024-yo}. Collectively, these efforts highlight MU’s growing role in building accountable and adaptable LLMs \citep{alsharabi}.


% Multilingual LLMs are designed to support multiple languages within a single architecture, facilitating knowledge transfer from high-resource to low-resource languages \cite{ye2023languageversatilistsvsspecialists, huang2025surveylargelanguagemodels}. Techniques for enhancing multilingual capabilities include training from scratch on balanced corpora, continued pretraining with language-specific adapters or tokens, and architectural modifications to support cross-lingual and culturally grounded reasoning \cite{wei2023polylmopensourcepolyglot, üstün2024ayamodelinstructionfinetuned}. Recent work has examined multilingual LLM performance in areas such as reasoning and hallucination \cite{chataigner2024multilingual}, as well as cultural understanding and localization \cite{culturalevaluating}.

% However, despite these advances, a critical gap remains in the domain of unlearning within multilingual LLMs. While unlearning has shown promise in monolingual settings for removing factual knowledge or mitigating harmful behaviors, its behavior across languages, especially in relation to culturally grounded content remains underexplored.

% Concurrently, growing attention has been paid to the presence of cultural and geopolitical biases in multilingual LLMs. Research has extended bias analyses beyond common axes such as gender and race to subtler cultural stereotypes, including nationality and regional representation \cite{kamruzzaman2024investigatingsubtlerbiasesllms}. For instance, \citet{li2024llmsidentifyculturalunity} and \citet{chiu2024culturalbenchrobustdiversechallenging} emphasize the need for robust cultural evaluation benchmarks (e.g., CulturalBench), while others demonstrate that current LLMs often fail to generate culturally appropriate or regionally nuanced responses \cite{dawson2024evaluatingculturalawarenessllms, rao-etal-2023-ethical}. To support more grounded evaluation, \citet{jha-etal-2023-seegull} introduce the SeeGULL dataset: a large-scale resource of geoculturally situated stereotypes spanning 178 countries and multiple regions.

% These findings underscore that multilingual capability alone is insufficient to ensure cultural fairness. Recent work \cite{liu2024multilingualllmsculturallydiversereasoners, singh2024translatingculturesllmsintralingual} further reveals LLMs' limitations in reasoning with culturally specific knowledge and adapting to local norms. As LLMs are deployed globally, addressing unlearning in this multilingual and multicultural context is both timely and necessary.




% ####################


% \begin{equation}
% \mathcal{L} = -\alpha_1 \cdot \mathcal{L}_\text{fgt} + \alpha_2 \cdot \mathcal{L}_\text{retain} + \alpha_3 \cdot \mathcal{L}_\text{nor}
% \label{eq:general}
% \end{equation}

% Here, $\mathcal{L}_\text{fgt}$ penalizes correct predictions on the forget set (e.g., stereotypical or sensitive answers), $\mathcal{L}_\text{retain}$ rewards correct behavior on the retain set, and $\mathcal{L}_\text{nor}$ is a KL divergence term that regularizes the updated model toward the original, preserving general capabilities. The weights $\alpha_1$, $\alpha_2$, and $\alpha_3$ control the trade-offs between forgetting, retention, and stability. In practice, the loss is adapted to the characteristics of each dataset, as described below.

% \begin{table}[ht]
% \centering
% \caption{\small Comparison of perplexity values for the fine-tuned Aya-Expanse-8B model and its unlearned variants across different languages.}
% \small
% \begin{tabular}{c|c}
% \toprule
% \textbf{Model Variant}        & \textbf{Perplexity} \\  
% \midrule \midrule
% Fine-tuned (All Langs)        & 23.15  \\
% Unlearned (English)           & 34.80  \\
% Unlearned (French)            & 44.12  \\
% Unlearned (Hindi)             & 40.04  \\
% Unlearned (Arabic)            & 43.82  \\
% Unlearned (Farsi)             & 45.64  \\
% \bottomrule
% \end{tabular}
% \label{tab:perplexity_results}
% \end{table}



% \begin{figure}[t]
%   \includegraphics[width=\columnwidth]{figures/prob_forget_plot_2e-5.png}
%   \caption{Prob. Forget for each of our 7 model, evaluated across all our 5 languages. A lower value is better, except for the finetune model. }
%   \label{fig:probforget}
% \end{figure}

% \begin{figure}[t]
%   \includegraphics[width=\columnwidth]{figures/truth_ratio_plot_2e-5.png}
%   \caption{Truth Ratio of the forget set for each of our 7 model, evaluated across all our 5 languages. A higher value is better. }
%   \label{fig:truthratio}
% \end{figure}


% \subsubsection{Evaluation}
% For TOFU, we follow the original evaluation framework \citep{tofu2024}, excluding ROUGE due to its limited applicability to languages like Arabic and Farsi. The evaluation is based on two key metrics: \textit{Probability} and \textit{Truth Ratio}. The probability metric estimates the model’s confidence in generating the correct answer $a$ given a question $q$, normalized by the answer length:

% \begin{equation}
% P(a \mid q)^{1/|a|},
% \end{equation}

% where $|a|$ denotes the number of tokens in the answer.

% The truth ratio measures how much more likely the model is to generate a paraphrased correct answer $\tilde{a}$ compared to perturbed incorrect variants $\hat{a} \in A_{\text{pert}}$:

% \begin{equation}
% \text{Truth Ratio} = \frac{1}{|A_{\text{pert}}|} \sum_{\hat{a} \in A_{\text{pert}}} \frac{P(\hat{a} \mid q)^{1/|\hat{a}|}}{P(\tilde{a} \mid q)^{1/|\tilde{a}|}}.
% \end{equation}

% We compute these metrics on the \textit{forget set} to evaluate unlearning, and on the \textit{retain set}, \textit{real authors}, and \textit{world facts} to assess model utility. The final utility score is the harmonic mean of all metrics on the three utility datasets.  To evaluate unlearning, we examine the probability
% and the truth ratio computed on the forget set.

% Furthermore, Table \ref{tab:perplexity_results} indicates the perplexity on test set of WikiText-2 benchmark \cite{wikitext} before and after unlearning for Aya model.



% \begin{table}[ht]
% \centering
% \small
% \resizebox{0.5\textwidth}{!}{
% \begin{tabular}{lccccc}
% \hline
%  & Model Utility & Prob. Retain & Prob. Forget & Truth Ratio Forget & Lang Distance \\
% \hline
% Model Utility        & 1.000 & 0.284 & -0.089 & -0.360 & 0.004 \\
% Prob. Retain         & 0.284 & 1.000 & 0.740  & -0.188 & 0.654 \\
% Prob. Forget         & -0.089 & 0.740 & 1.000  & -0.173 & 0.898 \\
% Truth Ratio Forget   & -0.360 & -0.188 & -0.173 & 1.000 & -0.293 \\
% Lang. Distance        & \textbf{0.004} & \textbf{0.654} & \textbf{0.898} & \textbf{-0.293} & \textbf{1.000} \\
% \hline
% \end{tabular}
% }
% \caption{Correlation between unlearning evaluation metrics and language distance.}
% \label{tab:correlation-metrics-distance}
% \end{table}

% f\subsubsection{Evaluation Metric}
% For SeeGULL, we evaluate the model on a modified QA dataset containing multiple-choice questions where one option reflects a stereotypical (harmful) response and another represents a neutral or ``Unknown'' response. Our primary unlearning metric is the reduction in selection of the stereotypical answer and an increase in the ``Unknown'' option after unlearning. This is a direct behavioral indicator of bias mitigation.

% To evaluate general model performance, we use the GLUE benchmark \citep{glue}, which comprises diverse natural language understanding tasks. We compare model accuracy on GLUE before and after unlearning to determine if our method adversely affects language capabilities. This two-fold evaluation ensures that unlearning stereotypical responses does not come at the cost of overall comprehension.

% This finding supports \textbf{RQ1}, indicating that unlearning in one language can influence others, especially when the base model is multilingual and trained with diverse sources.

==> latex/extra.tex <==
% In this work, we address the problem of multilingual unlearning by distinguishing between two key categories of information to be forgotten: (1) \textit{fine-tuned knowledge} and (2) \textit{biases inherited from pretraining corpora}. 
% Using the TOFU and SeeGULL datasets translated into English, French, Hindi, Arabic, and Farsi, we demonstrate that unlearning targeted content in one language generally results in minimal performance degradation in others. However, partial propagation occurs, particularly between typologically similar or high-resource languages such as English and French. 
% These findings underscore the need for language-aware unlearning strategies and the development of multilingual safety benchmarks that account for shared context and cross-lingual transfer effects.


% As multilingual large language models become increasingly prevalent, ensuring their safety and fairness across languages presents new challenges. While most machine unlearning research has focused on monolingual contexts, multilingual settings introduce unique complexities due to cross-lingual knowledge transfer and entrenched biases in both pretraining and fine-tuning data. In this work, we address the problem of multilingual unlearning by distinguishing between two key categories of information to be forgotten: (1) \textit{fine-tuned knowledge}—such as stereotypes introduced during downstream training—and (2) \textit{biases inherited from pretraining corpora}. We perform unlearning multilingual scenarios using the TOFU and SeeGULL datasets, translated into English, French, Hindi, Arabic, and Farsi. Our experiments demonstrate that unlearning targeted content in one language typically results in minimal performance degradation in others. However, partial propagation is observed, particularly between typologically or resource-similar languages like English and French. These findings highlight the need for language-aware unlearning strategies and the development of multilingual safety benchmarks that account for shared context and cross-lingual transfer effects.


% This task is known as \textbf{machine unlearning} and centers on deleting individual data points while preserving the model’s remaining knowledge \citep{bourtoule2021machine, zhang2024rightforgotteneralarge}.
% A separate challenge is eliminating broader unsafe or harmful content that the model has absorbed during pre-training, such as nationality-based slurs, self-harm instructions, or recipes for chemical weapons. Removing these high-level behaviors—often called \textbf{concept unlearning}—is motivated by safety and harm-reduction rather than privacy \citep{liu2024rethinkingmachineunlearninglarge}.
% Together, machine and concept unlearning provide complementary tools: the former enforces privacy compliance at the data-point level, while the latter mitigates harmful or dangerous behaviors embedded in the model’s general knowledge \citep{Jaman, NEURIPS2023_2ecc8008}.

% 
% Whenever these models memorize private facts, amplify defamation, or encode harmful stereotypes, developers must be able to delete that information quickly, reliably, and without the prohibitive cost of full retraining \citep{zhang2024rightforgotteneralarge}. This imperative, rooted in regulations such as the EU’s “Right to be Forgotten” and in growing safety concerns, has given rise to the field of machine unlearning: methods that remove selected knowledge while preserving the rest of the model’s capabilities. Early work on machine unlearning focused on efficiently excising particular training examples or data points from models \citep{bourtoule2021machine}. Since then, the scope of unlearning has expanded to include removing broader, potentially harmful concepts that a model may have inadvertently learned. In parallel, ensuring that LLMs avoid undesirable or unsafe behaviors, such as perpetuating cultural stereotypes learned during pretraining, has become a major challenge \citep{liu2024rethinkingmachineunlearninglarge}. Unlearning, therefore, plays a dual role: enabling \textit{privacy} (by removing personal or factual content) and promoting \textit{fairness} (by mitigating harmful social biases \citealp{Jaman, NEURIPS2023_2ecc8008}).
% In this paper, we take the first step towards filling that gap. We ask two concrete questions:
% \begin{itemize}
%     \item \textbf{RQ1:} If we unlearn something in one language, does it also disappear in other languages within the same multilingual model?
%     \item \textbf{RQ2:} How does the effect of unlearning vary across languages and types of information (fine-tuned vs. pretrained)? Is cross-lingual propagation more likely between linguistically similar or high-resource languages?
% \end{itemize}
% These questions matter not only for model safety, but also for efficient intervention. If forgetting generalizes across languages, we can apply targeted unlearning in just one or two languages. If not, multilingual unlearning requires language-specific solutions.

% To address these questions, we conduct two complementary experiments that correspond to the data and concept unlearning settings which we define in the Section~\ref{sec:methodology}.
% \begin{itemize}
%     \item \textbf{Data Unlearning}. To evaluate the removal of individual sensitive data points, we utilize the privacy-oriented TOFU benchmark \citep{tofu2024}, originally designed to assess factual unlearning in English. We extend this benchmark to four additional languages (French, Hindi, Arabic, and Farsi). This language set help us analysis how typological similarity (e.g., English–French) and resource availability (e.g., low-resource Farsi) influence the transferability of unlearning effects in multilingual LLMs.
%     \item \textbf{Concept Unlearnin}g. We assess the deletion of broader harmful concepts with a question-answering adaptation of SeeGULL \cite{jha-etal-2023-seegull} stereotype corpus, chosen for its fine-grained coverage of nationally anchored stereotypes.
%     % We release multilingual versions in English, French, and Hindi to capture both high- and mid-resource scenarios.
% \end{itemize}

% We propose the first framework to evaluate the transferability of unlearning in multilingual LLMs, addressing two key scenarios, machine unlearning and concept unlearning.
% \item \textbf{Multilingual Extension of Unlearning Benchmarks}: We extend two established unlearning benchmarks, TOFU and SeeGULL, to support multilingual evaluation across 5 languages. Our evaluation includes [human-verified translations / quality control] to ensure the reliability of multilingual data to enable accurate assessment of unlearning transferability across languages. (Clarify the annotation status here, if there’s no human annotation, we should not claim the translation quality or creation of the multilingual benchmark as a contribution.)


% To answer these questions, we study multilingual unlearning in LLMs by examining two distinct types of information:
% (1) Fine-tuned knowledge and
% (2) Pretraining-derived biases.
% For empirical analysis, we construct two complementary testbeds: a multilingual adaptation of the TOFU factual-forgetting benchmark (English, French, Hindi, Arabic, Farsi) and a question-answering version of the geo-cultural SeeGULL stereotype dataset. We then apply a gradient-ascent unlearning procedure that down-weights the probability of undesirable answers while maintaining performance on held-out data, and we measure cross-lingual effects on Aya-Expanse-8B and Llama-3.1-8B-Instruct.

% In this work, we study multilingual unlearning in LLMs by examining two distinct types of information: (1) \textit{fine-tuned knowledge}, such as stereotypes introduced during downstream training; and (2) \textit{biases inherited from pretraining data}, which are harder to localize and remove. We employ Gradient Ascent (GA) based approaches for unlearning, which allow us to target undesirable behaviors while preserving unrelated capabilities. To analyze cross-lingual effects, we use two multilingual datasets: the TOFU dataset \citep{tofu2024} for fact unlearning (translated into French, Hindi, Arabic, and Farsi), and an adapted version of the SeeGULL dataset \citep{jha-etal-2023-seegull} for stereotype unlearning across English, French, and Hindi. 
% % The SeeGULL dataset contains over 7,000 stereotypes from 178 countries, enabling us to probe geoculturally situated bias representations across languages.
% In our study we address the following research questions:
% \begin{itemize}
%     \item \textbf{RQ1:} Does unlearning in one language affect the same content in others? That is, is unlearning in one language sufficient to remove the corresponding information from the multilingual model?
%     \item \textbf{RQ2:} How does the effect of unlearning vary across languages and types of information (fine-tuned vs. pretrained)? Is cross-lingual propagation more likely between linguistically similar or high-resource languages?
% \end{itemize}

% These questions matter not only for model safety, but also for efficient intervention. If forgetting generalizes across languages, we can apply targeted unlearning in just one or two languages. If not, multilingual unlearning requires language-specific solutions.

% Our contributions are summarized as follows:
% \begin{itemize}
%     \item We present one of the \textbf{first} systematic studies of cross-lingual unlearning in multilingual LLMs, examining how unlearning in one language affects others.
%     % (Figure~\ref{fig:main})
%     \item We distinguish between fine-tuned knowledge and pretraining biases, showing they behave differently under unlearning interventions.
%     \item We adapt and utilize multilingual versions of the TOFU and SeeGULL datasets to support evaluation across privacy and fairness contexts.
%     \item We find that unlearning effects are often language-specific but can partially propagate between closely related or high-resource languages, such as English and French.
% \end{itemize}


% Recent advances in machine unlearning (MU) have shown promising potential for both privacy protection and bias mitigation in LLMs \citep{NEURIPS2023_2ecc8008, alsharabi}. Broadly, MU refers to the process of selectively removing training-induced knowledge such that the model behaves as if specific data were never seen. Initially introduced by \citet{cao}, the concept has evolved through techniques like sharded retraining, most notably the SISA framework, which enables efficient data deletion without full model retraining \citep{bourtoule2021machine} and selective forgetting via controlled parameter updates \citep{golatkar2020eternalsunshinespotlessnet}.

% More recently, MU has been applied to LLMs through two main approaches: fine-tuning-based unlearning such as gradient ascent to erase copyrighted or sensitive content \citep{eldan2023whosharrypotterapproximate, chen2023unlearnwantforgetefficient} and direct parameter editing via methods like weight surgery or subspace pruning \citep{meng2023locatingeditingfactualassociations, lizzo2024unlearnefficientremovalknowledge}. Additionally, \citet{Zhang2024-yo} demonstrate that unlearning biased data points can be achieved without introducing new biases, emphasizing MU’s potential for fairness. \citet{NEURIPS2023_2ecc8008} further propose a counterfactual unlearning approach using influence functions and minimal parameter updates to reduce the cost of retraining. Complementary to these, \citet{Yuanshun} show that using negative examples where models are fine-tuned to assign low likelihoods to harmful/undesired outputs, can outperform RLHF in safety alignment tasks, offering a more computationally efficient alternative.

% In recent years, MU has been extended to LLMs, giving rise to two main methodological paradigms: (1) fine-tuning-based unlearning, and (2) parameter-specific editing. In the first approach, models are subjected to additional fine-tuning that reverses or overwrites learned representations. For example, gradient ascent has been used to make models forget copyrighted material or sensitive information without requiring full retraining \citep{eldan2023whosharrypotterapproximate, chen2023unlearnwantforgetefficient}. In contrast, parameter-editing methods aim to directly identify and modify the weights responsible for encoding specific facts or behaviors. Techniques such as weight surgery and knowledge-subspace pruning have been proposed to surgically remove unwanted information while preserving general model performance \citep{meng2023locatingeditingfactualassociations, lizzo2024unlearnefficientremovalknowledge}.



%##############################


% Machine unlearning (MU) aims to remove the influence of specific training data from a model, ensuring it behaves as if that data were never seen \citep{cao}. Early frameworks such as SISA introduced sharded retraining for efficient data deletion \citep{bourtoule2021machine}, while later work proposed selective forgetting via parameter updates \citep{golatkar2020eternalsunshinespotlessnet}. More recently, MU has been applied to LLMs through two main approaches: fine-tuning-based unlearning such as gradient ascent to erase copyrighted or sensitive content \citep{eldan2023whosharrypotterapproximate, chen2023unlearnwantforgetefficient} and direct parameter editing via methods like weight surgery or subspace pruning \citep{meng2023locatingeditingfactualassociations, lizzo2024unlearnefficientremovalknowledge}.

% These strategies have shown promise in mitigating bias and enhancing safety. For instance, counterfactual unlearning based on influence functions has enabled low-cost updates with minimal side effects \citep{NEURIPS2023_2ecc8008}, while others leverage negative examples to suppress harmful outputs more efficiently than RLHF \citep{Yuanshun}. Further, unlearning biased samples without introducing new biases has been demonstrated as a pathway to fairer model behavior \citep{Zhang2024-yo}. Collectively, these efforts highlight MU’s growing role in building accountable and adaptable LLMs \citep{alsharabi}.


% Multilingual LLMs are designed to support multiple languages within a single architecture, facilitating knowledge transfer from high-resource to low-resource languages \cite{ye2023languageversatilistsvsspecialists, huang2025surveylargelanguagemodels}. Techniques for enhancing multilingual capabilities include training from scratch on balanced corpora, continued pretraining with language-specific adapters or tokens, and architectural modifications to support cross-lingual and culturally grounded reasoning \cite{wei2023polylmopensourcepolyglot, üstün2024ayamodelinstructionfinetuned}. Recent work has examined multilingual LLM performance in areas such as reasoning and hallucination \cite{chataigner2024multilingual}, as well as cultural understanding and localization \cite{culturalevaluating}.

% However, despite these advances, a critical gap remains in the domain of unlearning within multilingual LLMs. While unlearning has shown promise in monolingual settings for removing factual knowledge or mitigating harmful behaviors, its behavior across languages, especially in relation to culturally grounded content remains underexplored.

% Concurrently, growing attention has been paid to the presence of cultural and geopolitical biases in multilingual LLMs. Research has extended bias analyses beyond common axes such as gender and race to subtler cultural stereotypes, including nationality and regional representation \cite{kamruzzaman2024investigatingsubtlerbiasesllms}. For instance, \citet{li2024llmsidentifyculturalunity} and \citet{chiu2024culturalbenchrobustdiversechallenging} emphasize the need for robust cultural evaluation benchmarks (e.g., CulturalBench), while others demonstrate that current LLMs often fail to generate culturally appropriate or regionally nuanced responses \cite{dawson2024evaluatingculturalawarenessllms, rao-etal-2023-ethical}. To support more grounded evaluation, \citet{jha-etal-2023-seegull} introduce the SeeGULL dataset: a large-scale resource of geoculturally situated stereotypes spanning 178 countries and multiple regions.

% These findings underscore that multilingual capability alone is insufficient to ensure cultural fairness. Recent work \cite{liu2024multilingualllmsculturallydiversereasoners, singh2024translatingculturesllmsintralingual} further reveals LLMs' limitations in reasoning with culturally specific knowledge and adapting to local norms. As LLMs are deployed globally, addressing unlearning in this multilingual and multicultural context is both timely and necessary.




% ####################


% \begin{equation}
% \mathcal{L} = -\alpha_1 \cdot \mathcal{L}_\text{fgt} + \alpha_2 \cdot \mathcal{L}_\text{retain} + \alpha_3 \cdot \mathcal{L}_\text{nor}
% \label{eq:general}
% \end{equation}

% Here, $\mathcal{L}_\text{fgt}$ penalizes correct predictions on the forget set (e.g., stereotypical or sensitive answers), $\mathcal{L}_\text{retain}$ rewards correct behavior on the retain set, and $\mathcal{L}_\text{nor}$ is a KL divergence term that regularizes the updated model toward the original, preserving general capabilities. The weights $\alpha_1$, $\alpha_2$, and $\alpha_3$ control the trade-offs between forgetting, retention, and stability. In practice, the loss is adapted to the characteristics of each dataset, as described below.

% \begin{table}[ht]
% \centering
% \caption{\small Comparison of perplexity values for the fine-tuned Aya-Expanse-8B model and its unlearned variants across different languages.}
% \small
% \begin{tabular}{c|c}
% \toprule
% \textbf{Model Variant}        & \textbf{Perplexity} \\  
% \midrule \midrule
% Fine-tuned (All Langs)        & 23.15  \\
% Unlearned (English)           & 34.80  \\
% Unlearned (French)            & 44.12  \\
% Unlearned (Hindi)             & 40.04  \\
% Unlearned (Arabic)            & 43.82  \\
% Unlearned (Farsi)             & 45.64  \\
% \bottomrule
% \end{tabular}
% \label{tab:perplexity_results}
% \end{table}



% \begin{figure}[t]
%   \includegraphics[width=\columnwidth]{figures/prob_forget_plot_2e-5.png}
%   \caption{Prob. Forget for each of our 7 model, evaluated across all our 5 languages. A lower value is better, except for the finetune model. }
%   \label{fig:probforget}
% \end{figure}

% \begin{figure}[t]
%   \includegraphics[width=\columnwidth]{figures/truth_ratio_plot_2e-5.png}
%   \caption{Truth Ratio of the forget set for each of our 7 model, evaluated across all our 5 languages. A higher value is better. }
%   \label{fig:truthratio}
% \end{figure}


% \subsubsection{Evaluation}
% For TOFU, we follow the original evaluation framework \citep{tofu2024}, excluding ROUGE due to its limited applicability to languages like Arabic and Farsi. The evaluation is based on two key metrics: \textit{Probability} and \textit{Truth Ratio}. The probability metric estimates the model’s confidence in generating the correct answer $a$ given a question $q$, normalized by the answer length:

% \begin{equation}
% P(a \mid q)^{1/|a|},
% \end{equation}

% where $|a|$ denotes the number of tokens in the answer.

% The truth ratio measures how much more likely the model is to generate a paraphrased correct answer $\tilde{a}$ compared to perturbed incorrect variants $\hat{a} \in A_{\text{pert}}$:

% \begin{equation}
% \text{Truth Ratio} = \frac{1}{|A_{\text{pert}}|} \sum_{\hat{a} \in A_{\text{pert}}} \frac{P(\hat{a} \mid q)^{1/|\hat{a}|}}{P(\tilde{a} \mid q)^{1/|\tilde{a}|}}.
% \end{equation}

% We compute these metrics on the \textit{forget set} to evaluate unlearning, and on the \textit{retain set}, \textit{real authors}, and \textit{world facts} to assess model utility. The final utility score is the harmonic mean of all metrics on the three utility datasets.  To evaluate unlearning, we examine the probability
% and the truth ratio computed on the forget set.

% Furthermore, Table \ref{tab:perplexity_results} indicates the perplexity on test set of WikiText-2 benchmark \cite{wikitext} before and after unlearning for Aya model.



% \begin{table}[ht]
% \centering
% \small
% \resizebox{0.5\textwidth}{!}{
% \begin{tabular}{lccccc}
% \hline
%  & Model Utility & Prob. Retain & Prob. Forget & Truth Ratio Forget & Lang Distance \\
% \hline
% Model Utility        & 1.000 & 0.284 & -0.089 & -0.360 & 0.004 \\
% Prob. Retain         & 0.284 & 1.000 & 0.740  & -0.188 & 0.654 \\
% Prob. Forget         & -0.089 & 0.740 & 1.000  & -0.173 & 0.898 \\
% Truth Ratio Forget   & -0.360 & -0.188 & -0.173 & 1.000 & -0.293 \\
% Lang. Distance        & \textbf{0.004} & \textbf{0.654} & \textbf{0.898} & \textbf{-0.293} & \textbf{1.000} \\
% \hline
% \end{tabular}
% }
% \caption{Correlation between unlearning evaluation metrics and language distance.}
% \label{tab:correlation-metrics-distance}
% \end{table}

% f\subsubsection{Evaluation Metric}
% For SeeGULL, we evaluate the model on a modified QA dataset containing multiple-choice questions where one option reflects a stereotypical (harmful) response and another represents a neutral or ``Unknown'' response. Our primary unlearning metric is the reduction in selection of the stereotypical answer and an increase in the ``Unknown'' option after unlearning. This is a direct behavioral indicator of bias mitigation.

% To evaluate general model performance, we use the GLUE benchmark \citep{glue}, which comprises diverse natural language understanding tasks. We compare model accuracy on GLUE before and after unlearning to determine if our method adversely affects language capabilities. This two-fold evaluation ensures that unlearning stereotypical responses does not come at the cost of overall comprehension.

% This finding supports \textbf{RQ1}, indicating that unlearning in one language can influence others, especially when the base model is multilingual and trained with diverse sources.
